Toward Degree Bias in Embedding-Based Knowledge Graph Completion

A fundamental task for knowledge graphs (KGs) is knowledge graph completion (KGC). It aims to predict unseen edges by learning representations for all the entities and relations in a KG. A common concern when learning representations on traditional graphs is degree bias. It can affect graph algorithms by learning poor representations for lower-degree nodes, often leading to low performance on such nodes. However, there has been limited research on whether there exists degree bias for embedding-based KGC and how such bias affects the performance of KGC. In this paper, we validate the existence of degree bias in embedding-based KGC and identify the key factor to degree bias. We then introduce a novel data augmentation method, KG-Mixup, to generate synthetic triples to mitigate such bias. Extensive experiments have demonstrated that our method can improve various embedding-based KGC methods and outperform other methods tackling the bias problem on multiple benchmark datasets.

==> sections/ethics.tex <==

\section*{Ethics Statement}
Scientific work published at EMNLP 2022 must comply with the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL Ethics Policy}. We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).

==> sections/limitations.tex <==
\section*{Limitations}

KG-Mixup has a couple of limitations. One is that it our study of degree bias and proposed solution only applies to embedding-based knowledge graph techniques. As such, path-based techniques like NBFNet~\cite{zhu2021neural} are not considered. We expect to explore degree bias for path-based methods in future work. Second, we only studied the degree bias problem in the context of KGs for the task of knowledge graph completion. Future work can explore how degree bias effects other tasks (e.g. entity alignment~\cite{sun2020benchmarking}) and attempt to extend KG-Mixup to such tasks. 
